Distributed two-time-scale methods over clustered networks

In this paper, we consider consensus problems over a network of nodes, where the network is divided into a number of clusters. We are interested in the case where the communication topology within each cluster is dense as compared to the sparse communication across the clusters. Moreover, each cluster has one leader which can communicate with other leaders in different clusters. The goal of the nodes is to agree at some common value under the presence of communication delays across the clusters. Our main contribution is to propose a novel distributed two-time-scale consensus algorithm, which pertains to the separation in network topology of clustered networks. In particular, one scale is to model the dynamic of the agents in each cluster, which is much faster (due to the dense communication) than the scale describing the slowly aggregated evolution between the clusters (due to the sparse communication). We prove the convergence of the proposed method in the presence of uniform, but possibly arbitrarily large, communication delays between the leaders. In addition, we provided an explicit formula for the convergence rate of such algorithm, which characterizes the impact of delays and the network topology. Our results shows that after a transient time characterized by the topology of each cluster, the convergence of the two-time-scale consensus method only depends on the connectivity of the leaders. Finally, we validate our theoretical results by a number of numerical simulations on different clustered networks.

==> history/analysis.tex <==
\section{Main results}
In this section, we analyze the convergence properties of the proposed distributed two-time-scale methods under delays presented in the previous section. Specifically, our results show that under some proper choice of step size $\beta$ the nodes in the network reach a consensus exponentially fast. In addition, we provide an explicit formula to show the dependence of this convergence on the network topology and the constant delays $\tau$. We begin our analysis by introducing more notation. 

We denote by $\Wbf^{a} = [w_{ij}^{a}] \in \Rset^{|\Vcal^{a}|\times |\Vcal^{a}|}$ the weighted adjacency matrix corresponding to $\Gcal^{a}$ at cluster $\Ccal^{a}$. Similarly, let $\Vbf(k) = [v_{ab}(k)]\in \Rset^{r\times r}$ be the time-varying weighted adjacency matrix corresponding to the sequence of graphs $\{\Gcal_{C}(k)\}$ between the clusters. For convenience, we use the following notation
\begin{align*}
\Xbf^{a} \triangleq \left(\begin{array}{c}
(x_{1}^{a})^T    \\
\vdots\\
(x_{n}^{a})^T   
\end{array}\right) \in\Rset^{|\Vcal^{a}|\times d},\;\Xbf_{\ell} \triangleq \left(\begin{array}{c}
(x_{\ell}^{1})^T    \\
\vdots\\
(x_{\ell}^{r})^T   
\end{array}\right) \in\Rset^{r\times d}.   
\end{align*}
Using this notation, the matrix forms of \eqref{alg:follower} and \eqref{alg:leader} are given
\begin{align}
\begin{aligned}
\Xbf^{a}(k+1) &= \Wbf^{a}\Xbf^{a}(k),\qquad \forall a = 1,\ldots,r,\\
\Xbf_{\ell}(k+1) &= (1-\beta)\Xbf_{\ell}(k) + \beta \Vbf(k)\Xbf_{\ell}(k-\tau).
\end{aligned}\label{alg:matrix_form} 
\end{align}
In addition, we denote by $\1$ a vetor whose entries are all equal to the constant $1$. Finally, we denote by $\xbar^{a}\in\Rset^{d}$, $a = 1,\ldots,r$ and $\xbar_{\ell}\in\Rset^{d}$ the average of the row vectors of $\Xbf^{a}$ and $\Xbf^{\ell}$, respectively, i.e., 
\begin{align*}
\xbar^{a} = \frac{1}{|\Vcal^{a}|}\sum_{i\in\Vcal^{a}}x_{i}^{a}\;\text{ and }\; \xbar_{\ell} = \frac{1}{r}\sum_{a=1}^{r}x_{\ell}^{a}.
\end{align*}
Next, we make an assumption on $\Wbf^{a}$, $a= 1,\ldots,r$, and $\Vbf(k)$ which is standard in the consensus literature to guarantee the convergence of the nodes’ estimates to a consensus point \cite{Olfati-Saber2004}. The assumption given below also imposes a constraint on the communication between the followers at each cluster and between the leaders of the clusters, in which the nodes are only allowed to exchange messages with neighboring nodes, i.e., those directly connected to them. 
\begin{assump}\label{assump:W_follower}
$\Wbf^{a}$, $a = 1,\ldots,r$, is a doubly stochastic matrix, i.e., $\sum_{i}w_{ij}^{a} = \sum_{j}w_{ij}^{a} = 1.$ Moreover, $w_{ii}^{a} > 0$, $\forall i$, and $w_{ij}^{a} > 0$ if and ony if $(i,j)\in\Ecal^{a}$ otherwise $w_{ij}^{a} = 0$.
\end{assump}
\begin{assump}\label{assump:V_leader}
There exists a positive constant $\gamma$ such that $\Vbf(k)$ satisfies the following conditions for all $k\geq0$:
\begin{itemize}
\item[(a)] $v_{aa}(k)\geq\gamma,$ for all $a = 1,\ldots,r$.
\item[(b)] $v_{ab}(k)\in[\gamma,1]$ if $(a,b)\in\mathcal{N}_{a}^{C}(k)$ otherwise $v_{ab}(k)=0$.
\item[(c)] $\sum_{a=1}^{r} v_{ab}(k)=\sum_{b=1}^{r} v_{ab}(k)=1,$ for all $a,b$.
\end{itemize}
\end{assump}
In addition, we assume that the sequence of undirected graphs $\mathcal{G}^{C}(k) = (\mathcal{V}^{C},\mathcal{E}^{C}(k))$ is uniformly connected, formally stated as follows.
\begin{assump}\label{assump:BConnectivity}
There exists an integer $B\geq1$ such that the following graph is connected for all integers $\ell\geq0:$ 
\begin{equation}
(\mathcal{V}^{C},\mathcal{E}^{C}(\ell B)\cup \mathcal{E}^{C}(\ell B+1)\cup\ldots\cup \mathcal{E}^{C}((\ell +1)B-1)).
\end{equation}
\end{assump}
We note that this assumption is considerably weaker than requiring each $\mathcal{G}^{C}(k)$ to be connected for all $k\geq0$. By Assumption \ref{assump:W_follower} and since $\Gcal^{a}$ is connected, each $\Wbf^{a}$ has $1$ as the largest singular value. Let $\sigma_{a}$ be the second largest eigenvalue of $\Wbf^{a}$, which by the Perron-Frobenis theorem \cite{Ren2005} we have $\sigma_{a}\in (0,1)$. Similarly, we denote by $\sigma_{\Vbf(k)}$ the second largest singular value of $\Vbf(k)$. Furthermore, let $\delta_{C}$ be a parameter representing the spectral properties of the time-varying graph $\Gcal^{C}(k)$ defined as
\begin{align}
\delta_{C} \leq \min\,\left\{\,\left(1-\frac{1}{4r^3}\right)^{1/B}\,,\,\max_{k\geq 0}\sigma_{V}(\Vbf(k))\,\right\}.\label{notation:delta}
\end{align}
Assumptions \ref{assump:W_follower} and \ref{assump:BConnectivity} imply that $\delta_{C}\in(0,1)$.



% we denote by $\sigma_{\Vbf}\in(0,1)$ the second largest eigenvalue of $\Vbf$. Our first result in the following lemma is to show that the values of the followers in each cluster track the iterate of their leader. 
\begin{lem}\label{lem:consensus_follower}
The sequence $\{\Xbf^{a}(k)\}$ generated by \eqref{alg:matrix_form} satisfies
\begin{align}
\|\Xbf^{a}(k) - \xbar^{a}(k)^T\1\| \leq \sigma_{a}^{k}\|\Ybf^{a}(0)\|.   \label{lem:consensus_follower:ineq}
\end{align}
\end{lem}

\begin{proof}
For convenience, we denote by $\Ybf^{a} = \Xbf^{a} - (\xbar^{a})^T\1$. Since $\Wbf^{a}$ is a doubly stochastic matrix, using \eqref{alg:matrix_form} we have
\begin{align}
\xbar^{a}(k+1) = \frac{1}{|\Vcal^{a}|}\sum_{i\in\Vcal^{a}} = \xbar^{a}(k).\label{lem:consensus_follower:eq1a}     
\end{align}
By \eqref{alg:matrix_form} and \eqref{lem:consensus_follower:eq1a} we consider for each $a = 1,\ldots,r$
\begin{align*}
\Ybf^{a}(k+1) &= \Xbf^{a}(k+1) - \xbar^{a}(k+1)^T\1\\
&= \Wbf^{a}\Xbf^{a}(k) - \xbar^{a}(k)^T\1 = \Wbf^{a}\Ybf^{a}(k),
\end{align*}
which yields \label{lem:consensus_follower:ineq}, i.e.,
\begin{align*}
\|\Ybf^{a}(k+1)\| = \|\Wbf^{a}\Ybf^{a}(k)\| \leq \sigma_{a}\|\Ybf^{a}(k)\|\leq \sigma_{a}^{k+1}\|\Ybf^{a}(0)\|.   
\end{align*}
\end{proof}
We next study the consensus between the leaders under communication delays $\tau$. We note that under communication delays the estimate in \eqref{alg:leader} depends on the time interval $[k-\tau,k]$ for all $k\geq 0$. We, therefore, utilize the discrete-time variant of the $Gr\ddot{o}nwall$-$Bellman$ Inequality \cite{Khalil2002}, to hand such a dependence. The following theorem is to show that the leaders reach an agreement under some proper choice of step sizes. 

\begin{thm}\label{thm:leader_consensus}

\end{thm}

\begin{proof}
For convenience, we denote by $\Ybf_{\ell} = \Xbf_{\ell} - \xbar_{\ell}^T\1$. Since $\Vbf(k)$ satisfies Assumption \ref{assump:V_leader}(c), using \ref{alg:matrix_form} we have  
\begin{align*}
&\Ybf_{\ell}(k+1) = (1-\beta)\Xbf_{\ell}(k) + \beta\Vbf(k)\Xbf_{\ell}(k-\tau)\\
&\hspace{2cm} - (1-\beta)\xbar_{\ell}^T\1 + \beta \xbar_{\ell}(k-\tau)^T\1\\
&= (1-\beta)\Ybf_{\ell}(k) + \beta\Vbf(k)\Ybf_{\ell}(k-\tau)\\
&=(1-\beta)^{k+1}\Ybf_{\ell}(0) + \beta\sum_{t=0}^{k}V(t)\Ybf_{\ell}(t-\tau)(1-\beta)^{k-t},
\end{align*}
which implies that
\begin{align}
\|\Ybf_{\ell}(k+1)\| &\leq  (1-\beta)^{k+1}\|\Ybf_{\ell}(0)\|\notag\\ 
&\quad+ \beta\sum_{t=0}^{k}(1-\beta)^{k-t}\|V(t)\Ybf_{\ell}(t-\tau)\|.    \label{thm:leader_consensus:eq1}
\end{align}
\end{proof}


\begin{remark}
\end{remark}

==> history/prob.tex <==
\section{Distributed two-time-scale consensus methods}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{cluster_leader_followers_r.png}
    \caption{A network of $N$ nodes is partitioned into $r$ densely connected clusters. The clusters are connected through a line graph. \tdoan{Fix $\ell_{1}$ to $\ell^{1}$}}
    \label{fig:cluster}
\end{figure}
We consider a network of $N$ nodes divided into $r$ disjoint connected clusters $\Ccal^{a}$, $a=1,\ldots,r$. The communication pattern between nodes within each cluster $\Ccal^{a}$ is modeled by a densely connected and undirected graph $\Gcal^{a} = (\Vcal^{a},\Ecal^{a})$, where $\Vcal^{a}$ is the set of node indexes and $\Ecal^{a}$ is the set of edges. Thus, we have $\Vcal^{a}\cap\Vcal^{b} = \emptyset$ for all $a\neq b$ and $\sum_{a=1}^{r}|\Vcal^{a}| = N$, where $|\Vcal^{a}|$ denotes the cardinality of the set $\Vcal^{a}$. In addition, the communication between the nodes in different clusters is described by a sparse time-varying graph $\Gcal^{C}(k) = (\Vcal^{C},\{\Ecal^{C}(k)\})$, that is, $(i,j)\in\Ecal^{C}(k)$ if and only if the nodes $i$ and $j$ are in different clusters and there exists an edge between them at time $k$. We  assume that $|\Vcal^{a}\cap\Vcal^{C}| = 1$, $a=1,\ldots,r$, i.e., each cluster has only one node, called \textit{the leader} of $\Ccal^{a}$, that is connected to (some) leaders of other clusters. Similarly, we name other nodes as followers.  Finally, the $N$ nodes are connected by a graph $\Gcal = (\Vcal,\Ecal)$, where $\Vcal = \cup_{a=1}^{r}\Vcal^{a}$ and $\Ecal = \cup_{a=1}^{r}\Ecal^{a}\cup \Ecal^{C}$.    

An illustrative example of clustered networks is given in Fig. \ref{fig:cluster} where the nodes are divided into $r$ clusters. The connection between nodes in each cluster is modeled by a densely connected graph while each cluster $\Ccal^{a}$ has one leader $\ell^{a}$, $a = 1,\ldots,r$, connected to other leaders through a line graph (described by black edges).  A concrete motivating example for this problem is coordinated control of multirobot systems across long distances \cite{Magnus2020}. Since the spaces between robots grow, they experience greater communication delays. The presence of delays, if not properly addressed, may lead to oscillatory behaviors and even instabilities. Thanks to passivity-based methods, the the adverse effects of time delays are addressed. Due to scattering transformation concerns, this coordinated control algorithm may not be willing to show the convergence rate. Thus, a distributed two-time scale consensus algorithm seem to be a proper choice for this problem.





Our focus is to study the consensus problem over the clustered network $\Gcal$ under the presence of communication delays between the leaders of the clusters. Specifically, suppose that each node $i\in\Vcal$ is initialized with some arbitrary value $p_{i}$. This variable may encode the local information at each node in $\Gcal$, e.g., the position and velocity of a robot in networked formation control problems. The goal of the nodes is to cooperatively agree at some common value, i.e., they achieve a consensus. Since the graphs $\Gcal^{a}$ are dense while $\Gcal^{C}(k)$ is sparse, information shared between the nodes within each cluster is mixed much faster than the one between the clusters. For example, in Fig.\ \ref{fig:cluster} the rate of information sent from $\ell_{1}$ to its followers in $\Ccal^{1}$ is much faster than the time it gets to the nodes in $\Ccal^{r}$. To model this difference, we propose a novel distributed two-time-scale consensus method, where the updates of the followers in any cluster is implemented at a faster time-scale as compared to the one between the leaders of the clusters. In particular, for each cluster $\Ccal^{a}$ each follower $i\in\Vcal^{a}$ maintains  a variable $x_{i}^{a}$ and the leader maintains $x_{\ell}^{a}$, both are set at their initial values. The nodes in each $\Ccal^{a}$, $a = 1,\ldots,r$, then consider the following updates 
\begin{align}
x_{i}^{a}(k+1) &= \sum_{j\in\Ncal_{i}^{a}}w_{ij}^{a}x_{j}^{a}(k),\; \forall i\in \Vcal^{a} \text{ and } i \neq \ell\in\Vcal^{a},\label{alg:follower}\\
x_{\ell}^{a}(k+1) &= (1-\beta)x_{\ell}^{a}(k) + \beta \sum_{b\in\Ncal_{a}^{C}(k)}v_{ab}(k)x_{\ell}^{b}(k-\tau),\label{alg:leader}
\end{align}
where $\Ncal_{i}^{a}$ is the neighboring set of node $i$ in the cluster $\Ccal^{i}$ and $\Ncal_{a}^{C}(k)$ is the neighboring set of leader $a$ in the graph $\Gcal^{C}(k)$ of the clusters at time $k$. Moreover, $w_{ij}^{a}$ and $v_{ab}(k)$ are some positive (time-varying) weights, which will be specified shortly. Here, Eq.\ \eqref{alg:follower} is a consensus step between the followers in each cluster $\Ccal^{a}$ and Eq.\ \eqref{alg:leader} is the consensus step between the leaders of the clusters. Note that the updates of the followers may take into account the value of its leaders but not vice versa. Finally, the constant $\tau$ in \eqref{alg:leader} represents the communication delays in the information exchange between the leaders and $\beta$ is some proper step sizes to handle these delays. 

The motivation of these updates is explained as follows. 

\begin{remark}

\end{remark}














